LLM2Vec: Large Language Models Are Secretly Powerful Text Encoders

Large decoder-only language models (LLMs) are the state-of-the-art models on most of today's NLP tasks and benchmarks. Yet, the community is only slowly adopting these models for text embedding tasks, which require rich contextualized representations. In this work, we introduce LLM2Vec, a simple unsupervised approach that can transform any decoder-only LLM into a strong text encoder. LLM2Vec consists of three simple steps: 1) enabling bidirectional attention, 2) masked next token prediction, and 3) unsupervised contrastive learning. We demonstrate the effectiveness of LLM2Vec by applying it to 4 popular LLMs ranging from 1.3B to 8B parameters and evaluate the transformed models on English word- and sequence-level tasks. We outperform encoder-only models by a large margin on word-level tasks and reach a new unsupervised state-of-the-art performance on the Massive Text Embeddings Benchmark (MTEB). Moreover, when combining LLM2Vec with supervised contrastive learning, we achieve state-of-the-art performance on MTEB among models that train only on publicly available data (as of May 24, 2024). Our strong empirical results and extensive analysis demonstrate that LLMs can be effectively transformed into universal text encoders in a parameter-efficient manner without the need for expensive adaptation or synthetic GPT-4 generated data.

==> 1_Sections/results.tex <==
\section{Results}
We evaluate \model{} on Massive Text Embedding Benchmark (MTEB), a benchmark of 7 diverse embedding task categories covering a total of 56 embedding datasets. Since \model{} is an instruction-following encoder, following \citet{su-etal-2023-Instructor} and \citet{Wang2023-e5mistral}, we add dataset-specific instruction to MTEB. We keep the same instrcutions as in InstructOR~\cite{su-etal-2023-Instructor}. Since evaluating each model's checkpoint takes almost 1.5 days of running on 8 80GB A100 gpus, we take only 15 tasks, spanning over almost all task categories of MTEB for some of the evaluations. We report all the ablations \parishad{remove if ablations are on full-eval} and plots on this evaluation subset for the sake of time. Using this subset, the evaluation takes a few hours on 8 80GB A100 gpus. The list of evaluation task subsets is presented in \Cref{app:mteb-subset}.

\setcounter{subsection}{-1}
\subsection{MLM Pretraining Results}

\input{Tables/main_table}
\subsection{Main Results}
\Cref{tab:main_results} shows the performance of \model{} compared to existing relevant models. We observe that our proposed recipe performs promisingly compared to models trained on only publicly avilable data. \parishad{more explanation}

% \vspace{20pt}
% show bidirectional+mean works better even without any finetuning:\\
% TABLE 1: zeroshot performance on 15/56? tasks (if space, if not, appendix)
% \vspace{20pt}

% show the performance of our \model{} versus other existing methods on MTEB based on public data, instruction, etc:\\
% TABLE: \model{} vs other models on 56 tasks
% \vspace{20pt}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{p{15cm}}
%     \hline
%         show the impact of \\\hline
% mistral-7b: \{uni,bi\}, pool\{mean,eos,weighted\}, \{inst,no-inst\}, bs\{64,512\}, lora{8, 32}\\\hline
%     \end{tabular}
%     \caption{Ablation study of Mistral-7B-Instruct-v0.2 on MTEB benchmark. The best \model{} finetuning employs LoRA rank, alpha, dropour XXX, batch size 64, mean pooling, bidirectional connections for 3000 steps.}
%     \label{tab:mistral-ablation}
% \end{table*}
\input{Tables/ablation_table}

\subsection{Discussion}
The ablation study of the model design and training hyperparameter's choice for Mistral model are presented in \Cref{tab:ablation_results}. Experimental results show that while training with both causal and bidirectional connections lead to significant improvement on MTEB compared to zero-shot performance of the model, the model with bidirectional connections shows more promise. These results also confirms that bidirectional connections work better with mean and weighted-mean pooling compared to EOS pooling. This implies that the bidirectional information flow between tokens leads to better representation in all the tokens, hence having an embedding from the combination of all tokens leads to better performance than taking only one token. Moreover, these results show that although the models are trained with query and document instructions, interestingly, using the instruction-tuned version of the models or the base one does not have a huge impact on the performance.

\begin{table*}[t]
    \centering
    \begin{tabular}{p{15cm}}
    \hline
Show that everything still holds for smaller models:\\\hline
s-llama-1.3b: \{uni,bi\}, pool\{mean,eos,weighted\}, \{inst,no-inst\}, \{full,lora\}\\\hline
    \end{tabular}
    \caption{Ablation study of Sheared-Llama-1.3b on MTEB benchmark.}
    \label{tab:sllama-ablation}
\end{table*}




We further show in \Cref{tab:sllama-ablation} that the main findings of our recipe, still hold true for smaller models such as Sheared-Llama-1.3b. Moreover, we show the effectiveness of using PEFT instead of full finetuning when finetuning Sheared-Llama. This indicates that preserving the pre-trained weights of LLMs during the finetuning is important for text encoding tasks.  

We plot the embeddings of 100 random samples from pubmed and products reviews classification datasets in \Cref{fig:mistral_ret_cls_qualitative}. As illustrated, in pubmed asymmetric retrieval task, the distribution of queries and documents are different. However, in symmetric classification task, queries and documents are from the same domain and same classification label. It can be observed that with enabling bidirectional connections and mean pooling in the pretrained Mistral model, the embeddings are more spread out. Subsequently, comparing zeroshot performance of the models with the performance of trained model, queries and corresponding documents are mapped on each other perfectly, highlighting the impact of training.

% -----
% best Mistral (instruct, bs64, bi, probably mean, lr2e-5, r16, medi_ml_miracl, more_lora?)
% -----
% bi:
% uni
% uni+eos
% -----
% pooling:
% w. mean
% eos
% -----
% no-instruct
% -----
% bs:
% 256
% 512
% -----
% lora r:
% 8
% 32
% -----

% -----
% best S-llama (no-instruct, bs4, bi, probably mean, medi_ml_miracl, lr2e-5, r16)
% -----
% bi:
% uni
% uni+eos
% -----
% pooling:
% w. mean
% eos
% -----
% no-instruct
% -----
% bs:
% 16
% 32
% -----
% lora r:
% 8
% 32
% -----
% full
% -----

\begin{table*}[t]
    \centering
    \begin{tabular}{p{10cm}}
    \hline
    show the impact of training data on mistral:\\\hline
    TABLE: MEDI vs MED\_MIRACL vs MEDI\_ML\_MIRACL\\
    \hline
    \end{tabular}
    \caption{Ablation study of Sheared-Llama-1.3b on MTEB benchmark. This can be merged with \Cref{tab:ablation_results}}
    \label{tab:training-data-ablation}
\end{table*}
As described in \Cref{sec:data}, the main recipe includes training the LLM with multi-lingual MIRACL data addition to MEDI, the training data introduced by \citet{su-etal-2023-Instructor}. We augment MEDI with MIRACL as we realize that asymmetric datasets in MEDI may have been seen by powerful recent models such as Mistral, and hence, more difficult data was required. In \Cref{tab:training-data-ablation}, we present the importance of MIRACL data and show the importance of multi-lingual MIRACL data in the English MTEB evualuation benchmark.

% show the impact of model size:\\
% TABLE: Olmo-7b vs Olmo-1.3b --> Cannot show it because we cannot train olmo-7b with full ft
% \vspace{20pt}

Our experimental results in \Cref{plot:sample-efficiency} also demonstrate that the large language models are sample-efficient, meaning that they achieve X\% of their performance with only 500 steps of training, overally using 32,000 data samples. Training dataset is significantly smaller than what concurrent papers are using for training the models (e.g., around 2,000,000 samples addcites).
% to show the sample efficiency, we can show that the performance of \model{} when ch-3000 is almost the same as ch-large (8000), also compared to other models.\\
% PLOT or not to PLOT: comparing \model{} ch-best (1k,2k) with ch-8000 --> sample efficiency
This figure also highlights the fact that the model with bidirectional connections learns faster than the causal counterpart.
% Bi vs uni on ch-500 steps to show bi learns faster

\vaibhav{Should there be an experiment that shows that bidirectional models rely on contrastive pretraining? Instructor with T5 vs Instructor with GTR?}

% \begin{itemize}
%     \item bi vs uni
%     \item mean vs eos vs weighted mean
%     \item size (small vs large)
%     \item lora vs full finetuning: show lora is better than ft for s-llama --> it makes sense 
%     \item sample efficiency
%     \item show pretrained mistral with bi 
%     \item instruction-tuned model vs. non-instruction
%     \item tsne of text embeddings (uni-eos vs bi-mean) --> in section LLM2Vec
% \end{itemize}

\paragraph{Analysis of attention patterns}


\subsection{Limitations}

there do exist much smaller models with comparable performance, e.g. - GTE large has the same score on MTEB as us, and it is 330M in size, although with a much complex training regime. BGE has higher score than us and much smaller size

Embedding size is pretty big

Large encoder -> Inference latency



==> 2_Appendices/future_work.tex <==
%--------------------------------------
\section{Future work}
\label{sec:appendix:future_work}
%--------------------------------------

\mm{Collect ideas for future work here.}

==> 2_Appendices/more_llm2vec.tex <==
%--------------------------------------
\newpage
\section{More details on our implementation of LLM2Vec}
\label{sec:appendix:llm2vec}
%--------------------------------------

\mm{Provide LLM2Vec details here.}

==> 2_Appendices/more_related_work.tex <==
%--------------------------------------
\newpage
\section{Extended related work}
\label{sec:appendix:related-work}
%--------------------------------------

\mm{All related work that don't fit in the main paper should go here.}

==> Tables/ablation_table.tex <==
\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccc}
    \toprule
    \multicolumn{1}{l}{\multirow{2}{*}{\# of datasets $\rightarrow$}} & Retr. & Rerank. & Clust. & PairClass. & Class. & STS & Avg\\
    \multicolumn{1}{l}{}                                & 3     & 2     & 3          & 1      & 3    & 3    & 15  \\
    \midrule
    \multicolumn{1}{l}{medi-ml-miracl bi mean}  & 59.22  & 70.77  & 42.96  &  92.29  & 70.02  & 84.78 & 66.99 \\
    \midrule
    \multicolumn{9}{l}{\emph{Connections and Pooling}}        \\ \midrule
    \multicolumn{1}{l}{mistral medi-ml-miracl bi eos} & 59.40 & 71.07 & 43.39 & 86.27 & 70.38 & 85.83 & 67.03 \\
    \multicolumn{1}{l}{mistral medi-ml-miracl bi w-mean}  & 58.74 & 70.80 & 43.58 & 90.67 & 70.64 & 85.32 & 67.14 \\ 
    \multicolumn{1}{l}{mistral medi-ml-miracl uni eos}  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\ 
    \multicolumn{1}{l}{mistral medi-ml-miracl uni mean}  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\ 
    \multicolumn{1}{l}{mistral medi-ml-miracl uni w-mean}  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\ 
    \midrule
    \multicolumn{9}{l}{\emph{Instruction-tuned}}        \\ \midrule
    \multicolumn{1}{l}{no-instruct medi-ml-miracl bi mean} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \\
    \midrule
    \multicolumn{9}{l}{\emph{Hyperparameters}}        \\ \midrule
    \multicolumn{1}{l}{mistral medi-ml-miracl bi mean lora\_r-8} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
    \multicolumn{1}{l}{mistral medi-ml-miracl bi mean lora\_r-32} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
    \multicolumn{1}{l}{mistral medi-ml-miracl bi mean bs-256} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
    \multicolumn{1}{l}{mistral medi-ml-miracl bi mean bs-512} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
    \midrule
    \multicolumn{9}{l}{\emph{Training Data}}        \\ \midrule
    \multicolumn{1}{l}{mistral medi-eng-miracl bi mean} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
    \multicolumn{1}{l}{mistral medi bi mean} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Main Ablation table. mistral-7b: \{uni,bi\}, pool\{mean,eos,weighted\}, \{inst,no-inst\}, bs\{256,512\}, lora{8, 32}. \parishadsuggests{}{This table goes to the appendix and another one with MLM models comes instead.}}
    \label{tab:ablation_results}
\end{table*}

==> Tables/medi_supervised.tex <==
\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{\# of datasets} $\rightarrow$}} & \textbf{Retr}. & \textbf{Rerank.} & \textbf{Clust.} & \textbf{PairClass.} & \textbf{Class.} & \textbf{STS} & \textbf{Summ.} & \textbf{Avg} \\
    \multicolumn{1}{l}{} & 15     & 4     & 11   & 3      & 12    & 10  & 1    & 56  \\ 
    \midrule
    \texttt{MTEB leader-board results}\\\cmidrule{1-1}
    % \multicolumn{9}{l}{\emph{Supervised Models}}  \\ \midrule
    \multicolumn{1}{l}{SimCSE$_\text{bert-sup}$~\citep{Gao2021SimCSESC}}  &  21.8 & 47.5 & 33.4 & 73.7 & 67.3 & 79.1    &  23.3    &  48.7 \\
    \multicolumn{1}{l}{Contriever~\citep{Izacard2021TowardsUD}}   &  41.9 & 53.1 & 41.1 & 82.5 & 66.7 & 76.5 & 30.4 & 56.0 \\
    \multicolumn{1}{l}{GTR$_\text{xxl}$~\citep{Ni2021LargeDE}}   &  48.5 & 56.7 & 42.4 & 86.1 & 67.4 & 78.4 & 30.6 & 59.0 \\
    % 67.4  &  42.4   & 86.1   &  56.7   &  48.5  &  78.4   & 30.6  &  59.0 \\
    \multicolumn{1}{l}{Sentence-T5$_\text{xxl}$~\citep{ni2022sentence}}   &  42.2 & 56.4 & 43.7 & 85.1 & 73.4 & 82.6 & 30.1 & 59.5 \\
    % 73.4   &  43.7  &  85.1    &  56.4  & 42.2  & 82.6  & 30.1  &  59.5 \\
    \multicolumn{1}{l}{Instructor-xl} & 49.3 & 57.3 & 44.7 & 86.6 & 73.1 & 83.1 & 32.3 & 61.8\\
    \multicolumn{1}{l}{E5$_\text{large-v2}$~\citep{wang2022text}}     & 50.6 & 56.6 & 44.5 & 86.0 & 75.2 & 82.1 & 30.2 & 62.3 \\
    % 75.2  & 44.5  & 86.0  & 56.6  & 50.6  & 82.1 & 30.2  & 62.3   \\
    \multicolumn{1}{l}{GTE$_\text{large}$~\citep{li2023towards}}     & 52.2 & 59.1 & 46.8 &85.0 & 73.3 & 83.4 & 31.7 & 63.1 \\
    % 73.3  & 46.8  & 85.0   & 59.1  & 52.2   & 83.4  & 31.7  & 63.1   \\
    \multicolumn{1}{l}{BGE$_\text{large-en-v1.5}$~\citep{xiao2023c}}   & 54.3 & 60.0 & 46.1 &87.1 & 76.0 & 83.1 & 31.6 & 64.2 \\
    % 76.0  & 46.1  & 87.1  & 60.0  & 54.3  & 83.1  &  31.6 & 64.2  \\ \hline
    \multicolumn{1}{l}{E5$_\text{mistral-7b}$ + synthetic data only}  & 46.9 & 59.0 & 50.5 & 86.0 & 78.2 & 81.2 & 31.9 & 63.1 \\
    \multicolumn{1}{l}{E5$_\text{mistral-7b}$ + full data}  & 56.9 & 60.2 & 50.3 & 88.3 & 78.5 & 84.6 & 31.4 & 66.6 \\
    % \textbf{78.5}  & 50.3  & \textbf{88.3}  &  \textbf{60.2}  & \textbf{56.9}  & \textbf{84.6}  & 31.4 & \textbf{66.6} \\
    \multicolumn{1}{l}{E5$_\text{mistral-7b}$ + public data only}  & \\
    % 78.2 & \textbf{50.5} & 86.0 & 59.0 & 46.9 & 81.2 & 31.9 & 63.1  \\
    Echo mistral last (from table 2) & 55.5 & 58.1 & 46.3 & 87.3 & 77.4 & 82.6 & 30.7 & 64.7\\
    \midrule
    \multicolumn{9}{l}{Old results}        \\ \midrule
    \multicolumn{1}{l}{medi-ml-miracl sllama uni eos}  & % 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & \textbf{00.0} & 00.0 & node-2-scus -> nlp-gpu-2\\ 
     42.2 & 56.3 & 45.4 & 75.4 & 68.3 & 77.7 & 29.6 & 57.3 \\
    % /scratch/sentence-encoder-training/output_more_lora/medi_ret_ml_miraclx1_train_f-lora_m-instructor_Sheared-LLaMA-1.3B_p-eos_token_b-4_l-512_bidirectional-False_neg_gpu-False_swap_anchor-True_hard_neg_gpu-True_e-10_s-42_train_config-none_w-1000_lr-2e-05_lora_r-16/results/checkpoint-40000/
    \multicolumn{1}{l}{medi-ml-miracl sllama bi mean}  &  43.8 & 56.7 & 44.9 & 78.6 & 69.1 & 79.2 & 29.9 & 58.3 \\ 
    % /scratch/sentence-encoder-training/output_more_lora_after_mlm/medi_ret_ml_miraclx1_train_f-lora_m-instructor_Mistral-7B-Instruct-v0.2_p-mean_b-64_l-512_bidirectional-True_neg_gpu-False_swap_anchor-True_hard_neg_gpu-True_e-10_s-42_train_config-repllama-v2_w-200_lr-2e-05_lora_r-16/results/checkpoint-3000 
    \multicolumn{1}{l}{MLM-medi-ml-miracl sllama bi mean}  & 44.4 & 57 & 44.7 & 80.5 & 70.4 & 80.1 & 30 & 59 \\
    \multicolumn{1}{l}{medi-ml-miracl mistral uni eos}  & 51.15 & 60.37 & 48.42 & 82.11 & 72.75 & 81.89 & 29.22 & 62.66 \\ 
    % \multicolumn{1}{l}{medi-ml-miracl mistral uni mean}  & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & \textbf{00.0} & 00.0 & iad2 -> nlp-gpu-1\\ 
    % \multicolumn{1}{l}{medi-ml-miracl mistral uni w-mean}  & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & \textbf{00.0} & 00.0 & iad2 -> ?\\ 
    \multicolumn{1}{l}{medi-ml-miracl mistral bi mean}  & 51.8 & 60.6 & 49.0 & 83.9 & 71.9 & 82.7 & 30.3 & 63.0 \\ 
    \multicolumn{1}{l}{MLM-medi-ml-miracl mistral bi mean}  & 51.98 & 60.48 & 48.91 & 83.72 & 72.13 & 80.78 & 30.18 & 62.75 \\ \midrule
    % /scratch/sentence-encoder-training/output_more_lora_after_mlm/medi_ret_ml_miraclx1_train_f-lora_m-instructor_Mistral-7B-Instruct-v0.2_p-mean_b-64_l-512_bidirectional-True_neg_gpu-False_swap_anchor-True_hard_neg_gpu-True_e-10_s-42_train_config-repllama-v2_w-200_lr-2e-05_lora_r-16/results/checkpoint-3000/ 

    % new results go here
    \texttt{Sheared-LLaMA-1.3B}\\\cmidrule{1-1}
    uni wmean & \\
    bi mlm simcse mean &  51.5 & 55.6 & 43.2 & 85.8 &73 & 83.6 & 30.1 & 62\\
    \cmidrule{1-1}
    \texttt{Llama-2-7b-chat}\\\cmidrule{1-1}
    uni wmean & \\
    bi mlm simcse mean & 54.3 & 57.7 & 45 & 87.9 & 76.5 & 83.4 & 28.8 & 64 \\
    \cmidrule{1-1}
    \texttt{Mistral-7B-Instruct-v0.2}\\\cmidrule{1-1}
    uni wmean & 54.8 & 57.4 & 41.1 & 86 & 76 & 83.4 & 30.7 & 63.2\\
    bi mlm simcse mean &  56.1 & 58.8 & 45.6 & 88.1 & 76 & 83.8 & 30.4 & 64.7\\
    bi mlm-100-80 simcse mean & \\
    (medi) bi mlm simcse mean &  51.1 & 60.9 & 49.6 & 84.6 & 73.4 & 81.3 & 29.7 & 63.1 \\
    \bottomrule
     
    % /scratch/sentence-encoder-training/output_more_lora_after_mlm/medi_ret_ml_miraclx1_train_f-lora_m-instructor_Sheared-LLaMA-1.3B_p-mean_b-4_l-512_bidirectional-True_neg_gpu-False_swap_anchor-True_hard_neg_gpu-True_e-10_s-42_train_config-none_w-1000_lr-2e-05_lora_r-16/results/checkpoint-40000/
    \end{tabular}%
    }
    \caption{Dummy caption for main table. Supervised models. %{\color{red} Seperate this Table into Two Tables in different pages. One of the should focus on just unsupervised models, and the other supervised.}
    }
    \label{tab:main_results}
\end{table*}

==> Tables/mteb_subset.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ll}
    \toprule
    Category & Task \\ \toprule
    \multicolumn{1}{l}{\multirow{3}{*}{Retrieval}} & SciFact\\
    & ArguAna\\
    & NFCorpus\\ \midrule
    
    \multicolumn{1}{l}{\multirow{2}{*}{Reranking}} & SciDocsRR\\
    & StackOverflowDupQuestions\\ \midrule

    \multicolumn{1}{l}{\multirow{3}{*}{Clustering}} & BiorxivClusteringS2S\\
    & MedrxivClusteringS2S\\ 
    & TwentyNewsgroupsClustering \\ \midrule

    \multicolumn{1}{l}{\multirow{1}{*}{Pair Classification}} & SprintDuplicateQuestions\\ \midrule

    \multicolumn{1}{l}{\multirow{3}{*}{Classification}} & Banking77Classification\\
    & EmotionClassification\\ 
    & MassiveIntentClassification \\ \midrule

    \multicolumn{1}{l}{\multirow{3}{*}{STS}} & STS17\\
    & SICK-R\\ 
    & STSBenchmark \\
    \bottomrule
    \end{tabular}
    \caption{The subset of MTEB evaluation benchmark used in plots and ablation studies.}
    \label{tab:mteb-subset}
\end{table}

==> Tables/tsne_info.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c c p{12cm}}
    \toprule
       Category & Label & Review \\\midrule
       
       Movie & Negative & Poor Things simply just wasn't for me. I really don't like to say I hate a movie... so we'll just go with \"it wasn't for me\". I did appreciate the production design and performances, but a lot of the cinematography and writing/directing choices just didn't work for me. Just a little too weird for my tastes. And felt way too long. I wanted to like it so bad, and was so disappointed to find myself disliking it so much. I know it's been getting good reviews from most people - I'm in the minority here! So if you're interested, definitely check it out! I'm a huge supporter of going to see a film if you are interested in it and deciding for yourself how you feel!\\\midrule
       
       Movie & Positive & I saw this yesterday along with several other movies, that's why I'm reviewing the next day. Poor Things is very well-made, smoothly written throughout, with excellent cinematography, and a rivetingly bizarre experience that is so worthy of award recognition! It is dystopian vibe reminds me of Terry Gilliam's style. Yorgos is exceptional at his craft involving surgical creations, color palettes different from most, and enriching dialogue that is clever yet sometimes weird in all his movies. Emma Stone deserves praise and Willem Dafoe is master class as always. The film might not be for everyone but it's surely impressive and deserving of the 8.5 rating.\\\midrule

       Phone & Negative & Own an Apple 11 mini, broke the screen and forgot my passcode to my apple ID. So here is where the problems start, can't reset passcode because they want to send a verification code to my phone, which is now broken. Can't set a different phone to receive my verification and when given a code by email it sends a link to apple.com at which point I need to sign in to my account to input verification code, which I have no passcode for so have no access to. When I hit reset passcode the cycle begins again. So even if I get a new iPhone I can't use it because it won't accept service until I sign into my account, which I can't because I don't have passcode, and they will only send passcode to my broken phone, and the cycle repeats.\\\midrule

       Phone & Positive & The iPhone 11 is a big surprise, packing more advanced technology (namely in the camera capabilities and the processing power under the hood) at a lower cost than the iPhone XR's price in 2018. It combines a large 6.1-inch display with a premium-feeling body, and comes in an array of colors too.\\\bottomrule
       \toprule
       \multicolumn{2}{c}{Category} & \multicolumn{1}{l}{Instruction} \\\midrule
       \multicolumn{2}{c}{Classification} & \multicolumn{1}{l}{Represent the sentence for classification:} \\
       \multicolumn{2}{c}{STS} & \multicolumn{1}{l}{Represent the sentence for semantic textual similarity:} \\
       \bottomrule
    \end{tabular}
    \caption{The four reviews and instructions for the TSNE visualization. Instruction categories include Classification, STS, and no instruction.}
    \label{tab:custom-zeroshot-ablation}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{c c p{12cm}}
    \toprule
       Task & Type & Text \\\midrule
       
       Retrieval & Query & Represent the medicine question for retrieving relevant documents; New daily persistent headache: should migrainous features be incorporated?\\\midrule
       
       Retrieval & Document & Represent the medicine document for retrieval; International Classification of Headache Disorders (ICHD-2) criteria for new daily persistent headache (NDPH) require tension-type headache features. Many patients with 'new-onset persistent' headache fail to fulfil such criteria due to prominent migrainous features.We reviewed all NDPH patients in our headache clinic, using the definition of persistent headache < 3 days after onset for > 3 months. The patients were dichotomised: patients meeting ICHD-2 criteria (NDPH-S) and patients failing to meet ICHD-2 criteria due to prominent migrainous features (NDPH-M). All patients had completed a structured intake form including demographics, headache profiles, Beck Depression Inventory (BDI), Short Form 36 (SF-36) Health Survey, and Migraine Disability Assessment (MIDAS). A telephone interview was conducted for follow-up.A total of 92 NDPH patients were enrolled (59 (64.1\%) NDPH-M, 33 (35.9\%) NDPH-S). Between the two subgroups, the sociodemographics were indistinguishable, but the patients with NDPH-M had higher headache intensity, BDI scores, MIDAS scores, and lower scores of most SF-36 subscales. After an average of 2 years of follow-up, 57 (66\%) had a good outcome ($\geq$ 50\% reduction in headache frequency). Cox proportional analysis showed that disease duration $\leq$6 months and NDPH-S diagnosis predicted good outcomes.\\\midrule
       
       Classification & Query & Represent this sentence for classification: When it works, its awesome. But mine died after about 8 months of normal use. The thing is, its under warranty and they won't repair it, since we bought through amazon. And you only have 90 days.\\\midrule

       Classification & Document & Represent this sentence for classification: Not even 6 months and it no longer works. Just out of warranty. I tried to contact HP by email for warranty service but they weren't helpful. For now, I'll shell out more than \$250 at Best Buy - which includes an extended warrenty.\\
       \bottomrule
    \end{tabular}
    \caption{Examples of retrieval (pubmed) and classification (roducts reviews classification) datasets with corresponding instruction.}
    \label{tab:tsne-ret-cls}
\end{table*}


==> Tables/unsupervised_subset_results.tex <==
\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Our subset: \# of datasets} \textbf{$\rightarrow$}}} & \textbf{Retr.} & \textbf{Rerank.} & \textbf{Clust.} & \textbf{PairClass.} & \textbf{Class.} & \textbf{STS} & \textbf{Summ.} & \textbf{Avg}\\
    \multicolumn{1}{l}{} & 3     & 2     & 3   & 1      & 3    & 3  & 0    & 15  \\ 
    \midrule
    \texttt{Mistral-7B-Instruct-v0.2}\\\cmidrule{1-1}
    uni wmean & 18.9 & 50.8 & 24.7 & 54.2 & 63.8 & 61.0 & 0 & 44.0 \\
    bi mean mlm & 30.6 & 55.6 & 27.6 & 70.7 & 65.9 & 72.8 & 0 & 51.5 \\
    bi mean mlm simcse & 46.0 & 62.3 & 26.7 & 91.9 & 69.6 & 78.1 & 0 & 58.5\\
    echo & 27.9 & 58.6 & 29.2 & 79.6 & 69.1 & 77.8 & 0 & 53.9 \\\cmidrule{1-1}
    \texttt{S-llama}\\\cmidrule{1-1}
    \cmidrule{1-1}
    \texttt{Llama-2-7b}\\\midrule
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Their subset: \# of datasets} \textbf{$\rightarrow$}}} & \textbf{Retr.} & \textbf{Rerank.} & \textbf{Clust.} & \textbf{PairClass.} & \textbf{Class.} & \textbf{STS} & \textbf{Summ.} & \textbf{Avg}\\
    \multicolumn{1}{l}{} & 4     & 3     & 3   & 2      & 4    & 10  & 0    & 26  \\ 
    \midrule
    \texttt{Mistral-7B-Instruct-v0.2}\\\cmidrule{1-1}
    uni wmean & 7.5 & 50.6 & 24.7 & 63.3 & 69.5 & 58.6 & 0 & 47.9 \\
    bi mean mlm & 16.6 & 54.8 & 27.6 & 66.1 & 67.1 & 68.9 & 0 & 54.0 \\
    bi mean mlm simcse & 31.8 & 60.6 & 26.7 & 74.3 & 68.9 & 76.6 & 0 & 60.7 \\
    echo & 18.0 & 58.0 & 29.2 & 74.0 & 69.0 & 73.9 & 0 & 57.5\\\cmidrule{1-1}
    \texttt{S-llama}\\\cmidrule{1-1}
    \cmidrule{1-1}
    \texttt{Llama-2-7b}\\
    \bottomrule
    
    \end{tabular}
    }
    \caption{Comparison to Echo embeddings \citep{springer2024repetition} on a subset of the MTEB tasks. \mm{We will move this table to the Appendix eventually.} \parishadsuggests{}{Do we need this here? We have the same full-eval results in the main paper}}
    \label{tab:unsupervised_results}
\end{table*}
